Self-Diagnosing GAN: Diagnosing Underrepresented Samples in Generative Adversarial Networks

Despite remarkable performance in producing realistic samples, Generative Adversarial Networks (GANs) often produce low-quality samples near low-density regions of the data manifold, e.g., samples of minor groups. Many techniques have been developed to improve the quality of generated samples, either by post-processing generated samples or by pre-processing the empirical data distribution, but at the cost of reduced diversity. To promote diversity in sample generation without degrading the overall quality, we propose a simple yet effective method to diagnose and emphasize underrepresented samples during training of a GAN. The main idea is to use the statistics of the discrepancy between the data distribution and the model distribution at each data instance. Based on the observation that the underrepresented samples have a high average discrepancy or high variability in discrepancy, we propose a method to emphasize those samples during training of a GAN. Our experimental results demonstrate that the proposed method improves GAN performance on various datasets, and it is especially effective in improving the quality and diversity of sample generation for minor groups.

==> [NeurIPS 2021] Self-Diagnosing GAN/figures/25_gaussian/25_gaussian_arxiv.tex <==
\begin{figure*}[!tb]
\centering
	\subfloat[LDRM and generated samples\label{fig:25_gaussain_ldrm}]{\includegraphics[width=0.35\linewidth]{{figures/25_gaussian/new_ldrm.png}}} \qquad
    \subfloat[LDRM distribution and the number of high-quality samples over modes  \label{fig:25_gaussain_mode}]{\includegraphics[width=0.35\linewidth]{{figures/25_gaussian/25_gaussian_LDRM_orig_bar_total_v2.png}}}
    \caption{(a) Training dynamics of 25 Gaussians. The index of each mode is equal to $5x+y$ where the coordinates $(x,y)\in \{0,1,2,3,4\}^2$.  LDRM of training samples is recorded for each mode  with window $|T|=50$. Modes with high LDRM do not appear in the generated samples. (b) The empirical distribution of LDRM  (box plot) for each mode from  training samples, compared with the number of high-quality generated samples from each mode (blue).  LDRM can effectively detect dropped modes.}
    \label{fig:25_gaussian}
\end{figure*}

==> [NeurIPS 2021] Self-Diagnosing GAN/figures/celeba_high_low_images/supple_celeba_high.tex <==
\begin{figure}[!ht]
    \centering
    \subfloat[Samples with high LDRM ($k$=0)]{\includegraphics[width=0.3\linewidth]{figures/celeba_high_low_images/ldrm_55000_60000_64_high100.jpg}} \quad
    \subfloat[Samples with high LDRV ($k\to\infty$) ]{\includegraphics[width=0.3\linewidth]{figures/celeba_high_low_images/ldrv_55000_60000_64_high100.jpg}}\\
    %\subfloat[Samples with high disc. score ($k$ = 0.1)]{\includegraphics[width=0.3\linewidth]{figures/celeba_high_low_images/ldr_conf_01_55000_60000_64_high100.jpg}} \\
    \subfloat[Samples with high disc. score ($k$=0.3)]{\includegraphics[width=0.3\linewidth]{figures/celeba_high_low_images/ldr_conf_03_55000_60000_64_high100.jpg}} \quad
    \subfloat[Samples with high disc. score ($k$=0.5)]{\includegraphics[width=0.3\linewidth]{figures/celeba_high_low_images/ldr_conf_05_55000_60000_64_high100.jpg}}\quad
    \subfloat[Samples with high disc. score ($k$=1.0)]{\includegraphics[width=0.3\linewidth]{figures/celeba_high_low_images/ldr_conf_10_55000_60000_64_high100.jpg}}\\
    \subfloat[Samples with high disc. score ($k$=3.0)]{\includegraphics[width=0.3\linewidth]{figures/celeba_high_low_images/ldr_conf_30_55000_60000_64_high100.jpg}}\quad
    \subfloat[Samples with high disc. score ($k$=5.0)]{\includegraphics[width=0.3\linewidth]{figures/celeba_high_low_images/ldr_conf_50_55000_60000_64_high100.jpg}}\quad
    \subfloat[Samples with high disc. score ($k$=7.0)]{\includegraphics[width=0.3\linewidth]{figures/celeba_high_low_images/ldr_conf_70_55000_60000_64_high100.jpg}}
    \caption{CelebA samples with highest discrepancy scores on various $k$}
    \label{fig:CelebA_high_samples}
\end{figure}

==> [NeurIPS 2021] Self-Diagnosing GAN/figures/celeba_high_low_images/supple_celeba_low.tex <==
\begin{figure}[!ht]
    \centering
    \subfloat[Samples with low LDRM ($k$=0)]{\includegraphics[width=0.3\linewidth]{figures/celeba_high_low_images/ldrm_55000_60000_64_low100.jpg}} \quad
    \subfloat[Samples with low LDRV ($k\to\infty$)]{\includegraphics[width=0.3\linewidth]{figures/celeba_high_low_images/ldrv_55000_60000_64_low100.jpg}}\\
    %\subfloat[Samples with low disc. score ($k$ = 0.1)]{\includegraphics[width=0.3\linewidth]{figures/celeba_high_low_images/ldr_conf_01_55000_60000_64_low100.jpg}} \\
    \subfloat[Samples with low disc. score ($k$=0.3)]{\includegraphics[width=0.3\linewidth]{figures/celeba_high_low_images/ldr_conf_03_55000_60000_64_low100.jpg}}\quad
    \subfloat[Samples with low disc. score ($k$=0.5)]{\includegraphics[width=0.3\linewidth]{figures/celeba_high_low_images/ldr_conf_05_55000_60000_64_low100.jpg}}\quad
    \subfloat[Samples with low disc. score ($k$=1.0)]{\includegraphics[width=0.3\linewidth]{figures/celeba_high_low_images/ldr_conf_10_55000_60000_64_low100.jpg}}\\
    \subfloat[Samples with low disc. score ($k$=3.0)]{\includegraphics[width=0.3\linewidth]{figures/celeba_high_low_images/ldr_conf_30_55000_60000_64_low100.jpg}}\quad
    \subfloat[Samples with low disc. score ($k$=5.0)]{\includegraphics[width=0.3\linewidth]{figures/celeba_high_low_images/ldr_conf_50_55000_60000_64_low100.jpg}}\quad
    \subfloat[Samples with low disc. score ($k$=7.0)]{\includegraphics[width=0.3\linewidth]{figures/celeba_high_low_images/ldr_conf_70_55000_60000_64_low100.jpg}}
    \caption{CelebA samples with lowest discrepancy scores on various $k$}
    \label{fig:CelebA_low_samples}
\end{figure}

==> [NeurIPS 2021] Self-Diagnosing GAN/figures/celeba_samples.tex <==
\begin{figure*}[!htb]
\centering
\begin{tabular}{cc}
	\subfloat[Images with lowest disc. score \label{fig:celeba_small}]{\includegraphics[width=0.32\linewidth]{{figures/celeba_high_low_images/celeba-low100.jpg}}} &\\
  
	
    \subfloat[Images with highest disc. score \label{fig:celeba_large}]{\includegraphics[width=0.32\linewidth]{{figures/celeba_high_low_images/celeba-high100.jpg}}}&\\
    
    \subfloat[Generated samples\label{fig:celeba_gen}]{\includegraphics[width=0.32\linewidth]{{figures/celeba_high_low_images/celeba-generated_samples.jpg}}}&  
    \multirow{-12.8}{*}{    \subfloat[Historgram of pixel count over intensity level    \label{fig:celeba_histogram}]{\includegraphics[width=0.44\linewidth,height=0.32\linewidth]{{figures/celeba_high_low_images/celeba-histogram.jpg}}}}\\
    \end{tabular}
    \caption{Examples of CelebA training images with (a) lowest and (b) highest discrepancy scores, and (c) generated samples after Phase 1 (without weighted sampling). Generated samples resemble training images with lowest discrepancy score. (d) A smoothed histogram of the intensities for 100 samples per group.
    The intensity levels of RGB channels are concatenated, resulting in a total of $768=256\times3$ levels. 
    Images with the lowest scores (blue) and generated samples (green) have a similar distribution, while images with the highest scores (red) show a high discrepancy. 
    }
    \label{fig:celeba_samples}
\end{figure*}

==> [NeurIPS 2021] Self-Diagnosing GAN/figures/cifar10_high_low_images/supple_cifar10_high.tex <==
\begin{figure}[!ht]
    \centering
    \subfloat[Samples with high LDRM ($k$=0)]{\includegraphics[width=0.3\linewidth]{figures/cifar10_high_low_images/ldrm_35000_40000_64_high100.jpg}} \quad
    \subfloat[Samples with high LDRV ($k\to\infty$) ]{\includegraphics[width=0.3\linewidth]{figures/cifar10_high_low_images/ldrv_35000_40000_64_high100.jpg}}\\
    %\subfloat[Samples with high disc. score ($k$ = 0.1)]{\includegraphics[width=0.3\linewidth]{figures/cifar10_high_low_images/ldr_conf_01_35000_40000_64_high100.jpg}} \\
    \subfloat[Samples with high disc. score ($k$=0.3)]{\includegraphics[width=0.3\linewidth]{figures/cifar10_high_low_images/ldr_conf_03_35000_40000_64_high100.jpg}} \quad
    \subfloat[Samples with high disc. score ($k$=0.5)]{\includegraphics[width=0.3\linewidth]{figures/cifar10_high_low_images/ldr_conf_05_35000_40000_64_high100.jpg}}\quad
    \subfloat[Samples with high disc. score ($k$=1.0)]{\includegraphics[width=0.3\linewidth]{figures/cifar10_high_low_images/ldr_conf_10_35000_40000_64_high100.jpg}}\\
    \subfloat[Samples with high disc. score ($k$=3.0)]{\includegraphics[width=0.3\linewidth]{figures/cifar10_high_low_images/ldr_conf_30_35000_40000_64_high100.jpg}}\quad
    \subfloat[Samples with high disc. score ($k$=5.0)]{\includegraphics[width=0.3\linewidth]{figures/cifar10_high_low_images/ldr_conf_50_35000_40000_64_high100.jpg}}\quad
    \subfloat[Samples with high disc. score ($k$=7.0)]{\includegraphics[width=0.3\linewidth]{figures/cifar10_high_low_images/ldr_conf_70_35000_40000_64_high100.jpg}}
    \caption{CIFAR-10 samples with highest discrepancy scores on various $k$}
    \label{fig:CIFAR-10_high_samples}
\end{figure}

==> [NeurIPS 2021] Self-Diagnosing GAN/figures/cifar10_high_low_images/supple_cifar10_low.tex <==
\begin{figure}[!ht]
    \centering
    \subfloat[Samples with low LDRM ($k$=0)]{\includegraphics[width=0.3\linewidth]{figures/cifar10_high_low_images/ldrm_35000_40000_64_low100.jpg}} \quad
    \subfloat[Samples with low LDRV ($k\to\infty$) ]{\includegraphics[width=0.3\linewidth]{figures/cifar10_high_low_images/ldrv_35000_40000_64_low100.jpg}}\\
    %\subfloat[Samples with low disc. score ($k$ = 0.1)]{\includegraphics[width=0.3\linewidth]{figures/cifar10_high_low_images/ldr_conf_01_35000_40000_64_low100.jpg}} \\
    \subfloat[Samples with low disc. score ($k$=0.3)]{\includegraphics[width=0.3\linewidth]{figures/cifar10_high_low_images/ldr_conf_03_35000_40000_64_low100.jpg}} \quad
    \subfloat[Samples with low disc. score ($k$=0.5)]{\includegraphics[width=0.3\linewidth]{figures/cifar10_high_low_images/ldr_conf_05_35000_40000_64_low100.jpg}}\quad
    \subfloat[Samples with low disc. score ($k$=1.0)]{\includegraphics[width=0.3\linewidth]{figures/cifar10_high_low_images/ldr_conf_10_35000_40000_64_low100.jpg}}\\
    \subfloat[Samples with low disc. score ($k$=3.0)]{\includegraphics[width=0.3\linewidth]{figures/cifar10_high_low_images/ldr_conf_30_35000_40000_64_low100.jpg}}\quad
    \subfloat[Samples with low disc. score ($k$=5.0)]{\includegraphics[width=0.3\linewidth]{figures/cifar10_high_low_images/ldr_conf_50_35000_40000_64_low100.jpg}}\quad
    \subfloat[Samples with low disc. score ($k$=7.0)]{\includegraphics[width=0.3\linewidth]{figures/cifar10_high_low_images/ldr_conf_70_35000_40000_64_low100.jpg}}
    \caption{CIFAR-10 samples with lowest discrepancy scores on various $k$}
    \label{fig:CIFAR-10_low_samples}
\end{figure}

==> [NeurIPS 2021] Self-Diagnosing GAN/figures/cifar10_samples.tex <==
\begin{figure*}[!tb]
\centering
\begin{tabular}{cc}
	\subfloat[Images with lowest disc. score \label{fig:cifar10_small}]{\includegraphics[width=0.32\linewidth]{{figures/cifar10_high_low_images/cifar10-low100.jpg}}} &\\

    \subfloat[Images with highest disc. score \label{fig:cifar10_large}]{\includegraphics[width=0.32\linewidth]{{figures/cifar10_high_low_images/cifar10-high100.jpg}}}&\\

    \subfloat[Generated samples\label{fig:cifar10_gen}]{\includegraphics[width=0.32\linewidth]{{figures/cifar10_high_low_images/cifar10-generated_samples.jpg}}}&  \multirow{-12.8}{*}{    \subfloat[Histogram of pixel count over intensity level    \label{fig:cifar10_histogram}]{\includegraphics[width=0.44\linewidth,height=0.32\linewidth]{{figures/cifar10_high_low_images/cifar10-histogram.jpg}}}}\\
    \end{tabular}
    \caption{Training images with (a) lowest, (b) highest discrepancy scores, and (c) generated samples. Generated samples resemble training images with lowest score. (d) A smoothed histogram of the intensities for 100 samples per group.
    The intensity levels of RGB channels are concatenated, resulting in total  $768=256\times3$ levels. 
    Images with the lowest scores (blue) and generated samples (green) have a similar distribution, while images with the highest scores (red) show a high discrepancy. }
    \label{fig:cifar10_samples}
\end{figure*}

==> [NeurIPS 2021] Self-Diagnosing GAN/figures/color_mnist_samples_arxiv.tex <==
\begin{figure}[t]
    \subfloat[Training data \label{fig:color_mnist_samples_train}]{\includegraphics[width=0.315\linewidth]{{figures/color_mnist_train.jpg}}}
	\hspace{0.3em}
    \centering
	\subfloat[PacGAN\label{fig:color_mnist_samples_PAC}]{\includegraphics[width=0.315\linewidth]{{figures/color_mnist_pacgan_gen.jpg}}}
	\hspace{0.3em}
    \subfloat[DiaGAN (Ours) \label{fig:color_mnist_samples_ours}]{\includegraphics[width=0.315\linewidth]{{figures/color_mnist_diagan_gen.jpg}}}
    \caption{Generated samples in Colored-MNIST with the majority rate of 99\%. (a) Examples of training data (b) Samples from PacGAN. (c) Dia-GAN (Ours). Our method successfully generates samples with minor features, while  others fail, as in (b).}
    \label{fig:color_mnist_samples}
\end{figure}

==> [NeurIPS 2021] Self-Diagnosing GAN/figures/ldr_instability.tex <==
\begin{figure}[t]
    \centering
    \subfloat[\label{fig:LDR_instability}]{\includegraphics[width=0.35\linewidth]{{figures/ldr_eval_3idx.png}}} 
	\subfloat[\label{fig:LDR_plot}]{\includegraphics[width=0.65\linewidth]{{figures/ldr_instability2.png}}}
	\caption{(a) LDR values of three randomly chosen samples, (b) LDR values (left) and rankings (right) of 50 samples during training of CIFAR-10 on SNGAN~\cite{sngan}. The values are recorded every 100 steps from 30000 to 40000 epochs (total 100 times). LDR values are unstable during training, so it is hard to diagnose GAN training from the LDR of a particular training step. The level of fluctuations varies much over samples. %We propose to use statistics of 
	}\label{fig:LDR_inst}
\end{figure}

==> [NeurIPS 2021] Self-Diagnosing GAN/figures/minor_recall/minor_recall.tex <==
\begin{figure*}[t]
\centering
\begin{tabular}{ccc}
	\subfloat[Major\label{fig:color_mnist_major}]{\includegraphics[width=0.11\linewidth]{figures/minor_recall/red.png}} & 
	\subfloat[Minor\label{fig:color_mnist_minor}]{\includegraphics[width=0.11\linewidth]{figures/minor_recall/green.png}} &
	\\
	\subfloat[Major\label{fig:fmnist_major}]{\includegraphics[width=0.11\linewidth]{figures/minor_recall/mnist.png}} & 
	\subfloat[Minor\label{fig:fmnist_minor}]{\includegraphics[width=0.11\linewidth]{figures/minor_recall/fmnist.png}} &
% 	\hspace{1em}
    \multirow{-8.7}{*}{\subfloat[Partial Recall of major/minor groups vs. minority level \label{fig:recall_plot}]{\includegraphics[width=0.52\linewidth, height=0.22\linewidth]{figures/real_partial_recall_control.png}}}\\
    \end{tabular}
    \caption{Analysis on generated samples of GAN trained with (1) Single-mode Gaussian, (2) A mixture of MNIST (major) and FMNIST (minor), and (3) Colored MNIST with Red (major) and Green (minor) samples. (a) $\sim$ (d) show the examples of generated samples with major/minor features, and (e) shows the Partial Recall of major (dotted)/minor (solid) samples in each dataset on various minority levels. Both the sample quality and partial recall rate are higher for major groups.}
    \label{fig:minor_recall}
\end{figure*}

==> [NeurIPS 2021] Self-Diagnosing GAN/figures/weighted_sampling/weighted_sampling.tex <==
\begin{figure*}[htb!]
\centering
\begin{tabular}{cc}       
    %\subfloat{\includegraphics[scale=1]{figures/weighted_sampling/cifar10_original_background.png}} & \subfloat{\includegraphics[scale=1]{figures/weighted_sampling/cifar10_weighted_background.png}} \\
    \subfloat{\includegraphics[scale=0.5]{figures/weighted_sampling/celeba_original_minority.png}} & \subfloat{\includegraphics[scale=0.5]{figures/weighted_sampling/celeba_weighted_minority.png}} \\
    \subfloat{\includegraphics[scale=0.5]{figures/weighted_sampling/celeba_origianl_background.png}} & \subfloat{\includegraphics[scale=0.5]{figures/weighted_sampling/celeba_weighted_background.png}} \\ %\\
    (a) Generated samples with original sampling & (b) Generated samples with weighted sampling
\end{tabular}
%\caption{Comparison of generated samples with (a) original sampling and with (b) weighted sampling for CIFAR-10 and CelebA. Examples of CIFAR-10 images with brighter backgrounds for the weighted sampling scheme (1st row). CelebA samples with minor features such as accessaries including glasses or hats (2nd row) or with more unique backgrounds (e.g. with some letters in the background) for the weighted sampling scheme (3rd row).}
\caption{Comparison of generated samples with (a) original sampling and with (b) weighted sampling for CelebA dataset. Examples of generated images with minor features such as accessories including glasses or hats appeared by our method (1st row), or with more unique backgrounds (e.g. with some letters in the background) (2nd row).}
\label{fig:weighted_sampling}
\end{figure*}

==> [NeurIPS 2021] Self-Diagnosing GAN/tables/FFHQ_occ_pr.tex <==
\begin{table}[!tb]
\centering
\caption{FFHQ minor attribute analysis. O stands for the occurrence of minor attributes among the generated samples in percentage (\%) and R stands for the Partial Recall.}
\label{table:FFHQ_occ_pr}
\vspace{0.2em}
%\scalebox{0.9}{
\small
\begin{tabular}{c|cc|cc}
\toprule
\multirow{2}{*}{} &\multicolumn{2}{c|}{Vanilla}&\multicolumn{2}{c}{\textbf{Dia-GAN}}\\
\cmidrule{2-5}
& O $\uparrow$ & R $\uparrow$ & O $\uparrow$ & R $\uparrow$ \\
\midrule
Black (4.80\%) & \textbf{3.00\scriptsize{$\pm$0.13}} & 0.27\scriptsize{$\pm$0.03} & 2.99\scriptsize{$\pm$0.17} & \textbf{0.30\scriptsize{$\pm$0.01}} \\
Indian (2.08\%) & 0.81\scriptsize{$\pm$0.19} & 0.26\scriptsize{$\pm$0.03} & \textbf{1.16\scriptsize{$\pm$0.03}} & \textbf{0.30\scriptsize{$\pm$0.01}} \\
Middle eastern (4.04\%) & 3.18\scriptsize{$\pm$0.20} & 0.27\scriptsize{$\pm$0.04} & \textbf{3.49\scriptsize{$\pm$0.61}} & \textbf{0.31\scriptsize{$\pm$0.00}} \\
\bottomrule
\end{tabular}
%}
\end{table}

==> [NeurIPS 2021] Self-Diagnosing GAN/tables/FFHQ_race.tex <==
\begin{table}[!tb]
    \centering
    \caption{Ratio(\%) of race on the FFHQ dataset classified by the DeepFace architecture~\cite{deepface}.}
    \small
    \begin{tabular}{c|cccccc}
    \toprule
         Race & Asian & Black & Indian & Latino hispanic & Middle eastern & White \\
         \midrule
         Ratio(\%) & 19.38 & 4.80 & 2.08 & 10.83 & 4.04 & 58.87 \\
    \bottomrule
    \end{tabular}
    \label{tab:FFHQ_race}
\end{table}

==> [NeurIPS 2021] Self-Diagnosing GAN/tables/LDRM_LDRV_weighted_sampling.tex <==
\begin{table}[!h]
    \caption{FID for GAN using weighted sampling with LDRM and LDRV.}
    \label{Atable:LDRM_LDRV_weighted_sampling}
    \centering
    \small
    \begin{tabular}{c|c|c|c|c}
    \toprule
    & \textbf{Baseline} & \textbf{LDRM} & \textbf{LDRV} & \textbf{Dia-GAN(Ours)} \\
    \midrule
    FID for CIFAR-10 & 26.90\scriptsize{$\pm$0.90} & 19.80\scriptsize{$\pm$0.47} & 20.08\scriptsize{$\pm$0.67} & \textbf{19.66\scriptsize{$\pm$0.42}} \\
    \midrule
    FID for CelebA & 7.12\scriptsize{$\pm$0.27} & 7.46\scriptsize{$\pm$0.57} & 7.08\scriptsize{$\pm$0.75} & \textbf{6.70\scriptsize{$\pm$0.69}} \\
    \bottomrule
    \end{tabular}
\end{table}

==> [NeurIPS 2021] Self-Diagnosing GAN/tables/LDRV_detection.tex <==
\begin{table}[]
    \caption{AUROC of minority detection using LDRM and LDRV on Colored-MNIST with various majority rates.}
    % \small
    % \vspace{-0.5em}
    \centering
    %\scalebox{0.87}{
    %\tabcolsep=0.11cm
    \small
    \begin{tabular}{c|c|c|c|c}
    \specialrule{.1em}{.05em}{.05em}
    Majority rate & \textbf{99\%} & \textbf{97\%} & \textbf{95\%} & \textbf{90\%} \\
    \hline
    LDRM & \textbf{1.000} & 0.327 & 0.418  & 0.566\\
    \hline
    LDRV & 0.172 & \textbf{0.997} & \textbf{0.999} & \textbf{0.992}\\
    \specialrule{.1em}{.05em}{.05em}
    \end{tabular}
    %}
   % \vspace{-0.5\baselineskip}

    \label{table:ldrv_detection}
%    \vspace{-0.5em}
\end{table}

==> [NeurIPS 2021] Self-Diagnosing GAN/tables/celeba_attribute_count_ldrv.tex <==
\newcolumntype{?}{!{\vrule width 0.8pt}}

\begin{table}[!tb]
\centering
\caption{CelebA minor attribute analysis. Averaged LDRV and averaged discrepancy score of CelebA samples with (W/) or without (W/O) minor attributes. O stands for the occurrence of minor attributes among the generated samples in percentage (\%) and R stands for the Partial Recall.}
\label{table:celeba_attr_count_ldrv}
\vspace{0.2em}
%\scalebox{0.9}{
\begin{tabular}{c?cc|cc?cc|cc}
\toprule
\multirow{3}{*}{} &\multicolumn{4}{c?}{Score}&\multicolumn{4}{c}{Method}\\
\cmidrule{2-9}
&\multicolumn{2}{c|}{LDRV }&\multicolumn{2}{c?}{Discrepancy }&\multicolumn{2}{c|}{Vanilla} &\multicolumn{2}{c}{\textbf{Dia-GAN}}\\
\cmidrule{2-9}
& W/ & W/O & W/ & W/O & O $\uparrow$ & R $\uparrow$ & O $\uparrow$ & R $\uparrow$ \\
\midrule
Bald (2.244\%) & \textbf{0.271} & 0.184 & \textbf{2.938} & 2.221& 0.678 & 0.353 & \textbf{0.836} & \textbf{0.393} \\
%\midrule
Double Chin (4.669\%) & \textbf{0.219} & 0.184 & \textbf{2.525} & 2.224 & 0.440 & 0.411 & \textbf{0.522} & \textbf{0.461}\\
%\midrule
Eyeglasses (6.512\%) & \textbf{0.254} & 0.181 & \textbf{2.783} & 2.200 & 3.300 & 0.400 & \textbf{4.053} & \textbf{0.449}\\
%\midrule
Gray Hair (4.195\%) & \textbf{0.211} & 0.185 & \textbf{2.450} & 2.228 & 2.273 & 0.402 & \textbf{2.369} & \textbf{0.436}\\
Mustache (4.155\%) & \textbf{0.242} & 0.183 & \textbf{2.699} & 2.218 & 0.157 & 0.391 & \textbf{0.228} & \textbf{0.433}\\
%\midrule
Pale Skin (4.295\%) & \textbf{0.190} & 0.186 & \textbf{2.240} & 2.238 & 0.346 & 0.380 & \textbf{0.453} & \textbf{0.427}\\
%\midrule
Wearing Hat (4.846\%) & \textbf{0.357} & 0.177 & \textbf{3.651} & 2.164 & 2.307 & 0.380 & \textbf{3.595} & \textbf{0.408}\\
\bottomrule
\end{tabular}
%}
\end{table}

==> [NeurIPS 2021] Self-Diagnosing GAN/tables/celeba_fid_full.tex <==
\begin{table}[h]
\centering
\caption{(Details of Table~\ref{table:cifar10-celeba-results}) Comparison of diverse sampling/weighting techniques for CelebA image generation.} 
\label{table:celeba-fid_pr_arxiv}
\vspace{1em}
\begin{tabular}{c|ccc|ccc}
\toprule
\multirow{2.5}{*}{Methods} &\multicolumn{3}{c|}{SNGAN}&\multicolumn{3}{c}{SSGAN}\\
\cmidrule{2-7}
& \textbf{FID $\downarrow$}  & \textbf{Prec. $\uparrow$} & \textbf{Rec. $\uparrow$} & \textbf{FID $\downarrow$}  & \textbf{Prec. $\uparrow$} & \textbf{Rec. $\uparrow$}\\
\midrule
Vanilla & 7.12\scriptsize{$\pm$0.27} & 0.68\scriptsize{$\pm$0.00}  & 0.44\scriptsize{$\pm$0.01} & 7.19\scriptsize{$\pm$0.18} & 0.68\scriptsize{$\pm$0.01} & 0.44\scriptsize{$\pm$0.02} \\
DRS~\cite{DRS} & 7.04\scriptsize{$\pm$0.31} & 0.68\scriptsize{$\pm$0.01} & 0.44\scriptsize{$\pm$0.01} & 7.08\scriptsize{$\pm$0.23} & 0.68\scriptsize{$\pm$0.01} & 0.45\scriptsize{$\pm$0.01}\\
GOLD~\cite{GOLD} & 7.31\scriptsize{$\pm$0.67} & \textbf{0.69\scriptsize{$\pm$0.00}} & 0.44\scriptsize{$\pm$0.02} & 7.46\scriptsize{$\pm$0.31} & 0.68\scriptsize{$\pm$0.00} & 0.43\scriptsize{$\pm$0.00}\\
GOLD + DRS~\cite{DRS} & 6.97\scriptsize{$\pm$0.64} & 0.68\scriptsize{$\pm$0.01} & 0.44\scriptsize{$\pm$0.01} & 7.15\scriptsize{$\pm$0.37} & 0.67\scriptsize{$\pm$0.01} & 0.45\scriptsize{$\pm$0.01}\\
Top-k~\cite{sinha2020top} & 7.35\scriptsize{$\pm$0.20} & 0.67\scriptsize{$\pm$0.00} & 0.44\scriptsize{$\pm$0.01} & 7.23\scriptsize{$\pm$0.18} & 0.67\scriptsize{$\pm$0.00} & 0.45\scriptsize{$\pm$0.01}\\
Top-k + DRS~\cite{DRS} & 7.35\scriptsize{$\pm$0.18} & 0.68\scriptsize{$\pm$0.00} & 0.44\scriptsize{$\pm$0.00} & 7.16\scriptsize{$\pm$0.25} & \textbf{0.68\scriptsize{$\pm$0.00}} & 0.45\scriptsize{$\pm$0.00}\\
\textbf{Dia-GAN} & \textbf{6.70\scriptsize{$\pm$0.69}} & 0.64\scriptsize{$\pm$0.02} & \textbf{0.48\scriptsize{$\pm$0.02}} & \textbf{6.88\scriptsize{$\pm$0.58}} & 0.66\scriptsize{$\pm$0.02} & \textbf{0.46\scriptsize{$\pm$0.02}}\\
\bottomrule
\end{tabular}
\end{table}


==> [NeurIPS 2021] Self-Diagnosing GAN/tables/cifar10_celeba_fid.tex <==
\begin{table}[t]
\centering
\caption{Comparison of diverse sampling/weighting methods for CIFAR-10/CelebA image generation.}
\label{table:cifar10-celeba-results}
\vspace{0.2em}
%\scalebox{0.9}{
\begin{tabular}{c|cc|cc|ccc|ccc}
\toprule
Dataset & \multicolumn{4}{c|}{CIFAR-10} & \multicolumn{6}{c}{CelebA}\\
\midrule
\multirow{2.5}{*}{Methods} &\multicolumn{2}{c|}{SNGAN}&\multicolumn{2}{c|}{SSGAN}&\multicolumn{3}{c|}{SNGAN}&\multicolumn{3}{c}{SSGAN}\\
\cmidrule{2-11}
& FID $\downarrow$    &IS $\uparrow$  & FID $\downarrow$    & IS $\uparrow$ & FID $\downarrow$  & P $\uparrow$ & R $\uparrow$ & FID $\downarrow$  & P $\uparrow$& R $\uparrow$ \\
\midrule
Vanilla & 26.90 & 7.36 & 22.01 & 7.65& 7.12 & 0.68  & 0.44& 7.19 & 0.68 & 0.44\\
DRS~\cite{DRS} & 24.54 & 7.57 & 20.51 & 7.77 & 7.04 & 0.68 & 0.44& 7.08 & 0.68 & 0.45\\
GOLD~\cite{GOLD} & 28.86 & 7.21 & 21.90 & 7.57 & 7.31 & \textbf{0.69} & 0.44& 7.46 & 0.68 & 0.43\\
GOLD + DRS & 24.65 & 7.53 & 19.36 & 7.79 & 6.97 & 0.68 & 0.44 & 7.15 & 0.67 & 0.45\\
Top-k~\cite{sinha2020top} &  24.45 &  7.60 & 20.01 & 7.78  & 7.35 & 0.67 & 0.44& 7.23 & 0.67 & 0.45\\
Top-k + DRS &  23.92 &  7.70 & 20.09 & 7.88 & 7.35 & 0.68 & 0.44 & 7.16 & \textbf{0.68} & 0.45\\
\textbf{Dia-GAN} & \textbf{19.66} & \textbf{7.95}& \textbf{16.31} & \textbf{8.14} & \textbf{6.70} & 0.64 & \textbf{0.48}& \textbf{6.88} & 0.66 & \textbf{0.46}\\
\bottomrule
\end{tabular}
%}
\end{table}


==> [NeurIPS 2021] Self-Diagnosing GAN/tables/cifar10_fid_full.tex <==
\begin{table}[h]
\centering
\caption{(Details of Table~\ref{table:cifar10-celeba-results}) Comparison of diverse sampling/weighting techniques for CIFAR-10 image generation.}
\label{table:cifar10-fid_is_arxiv_v2}
\vspace{1em}
\begin{tabular}{c|cc|cc}
\toprule
\multirow{2.5}{*}{Methods} &\multicolumn{2}{c|}{SNGAN} &\multicolumn{2}{c}{SSGAN}\\
\cmidrule{2-5}
& \textbf{FID $\downarrow$}    & \textbf{IS $\uparrow$} & \textbf{FID $\downarrow$} & \textbf{IS $\uparrow$}\\
\midrule
Vanilla & 26.90\scriptsize{$\pm$0.90} & 7.36\scriptsize{$\pm$0.08} & 22.01\scriptsize{$\pm$0.99} & 7.65\scriptsize{$\pm$0.10}\\
DRS~\cite{DRS} & 24.54\scriptsize{$\pm$0.80} & 7.57\scriptsize{$\pm$0.05} & 20.51\scriptsize{$\pm$1.01} & 7.77\scriptsize{$\pm$0.09} \\
GOLD~\cite{GOLD} & 28.86\scriptsize{$\pm$0.92} & 7.21\scriptsize{$\pm$0.09} & 21.90\scriptsize{$\pm$0.90} & 7.57\scriptsize{$\pm$0.09} \\
GOLD + DRS~\cite{DRS} & 24.65\scriptsize{$\pm$0.86} & 7.53\scriptsize{$\pm$0.09} & 19.36\scriptsize{$\pm$0.45} & 7.79\scriptsize{$\pm$0.04} \\
Top-k~\cite{sinha2020top} &  24.45\scriptsize{$\pm$0.60} &  7.60\scriptsize{$\pm$0.06} & 20.01\scriptsize{$\pm$1.23} & 7.78\scriptsize{$\pm$0.08} \\
Top-k + DRS~\cite{DRS} &  23.92\scriptsize{$\pm$0.69} &  7.70\scriptsize{$\pm$0.09} & 20.09\scriptsize{$\pm$0.98} & 7.88\scriptsize{$\pm$0.10} \\
\textbf{Dia-GAN} & \textbf{19.66\scriptsize{$\pm$0.42}} & \textbf{7.95\scriptsize{$\pm$0.09}} & \textbf{16.31\scriptsize{$\pm$0.53}} & \textbf{8.14\scriptsize{$\pm$0.06}} \\
\bottomrule
\end{tabular}
\end{table}


==> [NeurIPS 2021] Self-Diagnosing GAN/tables/controlled_re.tex <==
\begin{table}[!tb]
\centering
\caption{Reconstruction Error (RE) score of green (minor) training samples in Colored MNIST and FMNIST (minor) samples in a mixture of MNIST and FMNIST on different majority rate $\rho$.}
\label{table:controlled_recon}
\vspace{0.2em}
\begin{tabular}{c|ccc|ccc}
\toprule
Dataset & \multicolumn{3}{c|}{Colored MNIST} & \multicolumn{3}{c}{MNIST-FMNIST}\\
\midrule
Majority rate $\rho$ &{99\%} &{95\%} &{90\%}  &{99\%} &{95\%} &{90\%}\\
\midrule
% Baseline & 0 & 680.46 & 70.5 & 53.73 & 64.09 & 47.48 \\
% GOLD~\cite{GOLD} & 0 & 678.83 & & 46.83 & & 47.78 \\
% Top-k~\cite{sinha2020top} & 0 & 681.42 & & 53.47 & & 51.28 \\
% PacGAN~\cite{lin2020pacgan} & 0 & 677.24 & & 55.66 & & 44.02 \\
% Inclusive GAN~\cite{InclusiveGAN} & 0 & 679.79 & & 52.71 && \textbf{34.89} \\
Vanilla & 0.838  & 0.236  & 0.218 & 0.290 & 0.227 & 0.215\\
GOLD~\cite{GOLD}  & 0.813 & 0.297 & 0.200 & 0.296 & 0.241 & 0.218 \\
Top-k~\cite{sinha2020top}  & 0.831  & 0.210  & 0.223 & 0.281 & 0.232 & 0.221\\
PacGAN~\cite{lin2020pacgan}  & 0.810  & 0.244  & 0.233 & 0.313 & 0.251 & 0.225\\
Inclusive GAN~\cite{InclusiveGAN} & 0.812 & 0.274 & 0.216 & 0.283 & 0.230 & 0.220 \\
\textbf{Dia-GAN}  & \textbf{0.224}&  \textbf{0.204} & \textbf{0.197} & \textbf{0.264} & \textbf{0.219} & \textbf{0.206}\\
\bottomrule
\end{tabular}
\end{table}

==> [NeurIPS 2021] Self-Diagnosing GAN/tables/dcgan_discriminator.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{table}[ht]
    \caption{Discriminator architecture for Colored MNIST \& MNIST-FMNIST}
    \label{table:dcgan_disc}
    \centering
    \small
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \toprule
    \multicolumn{8}{c}{\textbf{Discriminator}} \\
    \midrule
    Layer & Output size & Kernel size & Stride & Padding & Batch Norm & Dropout & Activation \\
    \midrule
    Input $x$ & 32$\times$32$\times \texttt{nc}$ &     &   &   &   &  \\
    Conv & 16$\times$16$\times$16 & 3$\times$3 & 2 & 1 & X & 0.5 & LeakyReLU(0.2) \\
    Conv & 16$\times$16$\times$32 & 3$\times$3 & 1 & 1 & O & 0.5 & LeakyReLU(0.2) \\
    Conv & 8$\times$8$\times$64 & 3$\times$3 & 2 & 1 & O & 0.5 & LeakyReLU(0.2) \\
    Conv & 8$\times$8$\times$128 & 3$\times$3 & 1 & 1 & O & 0.5 & LeakyReLU(0.2) \\
    Conv & 4$\times$4$\times$256 & 3$\times$3 & 2 & 1 & O & 0.5 & LeakyReLU(0.2) \\
    Conv & 4$\times$4$\times$512 & 3$\times$3 & 1 & 1 & O & 0.5 & LeakyReLU(0.2) \\
    Flatten & - & - & - & - & - & - & - \\
    FC & 1  & - & - & - & X & & Sigmoid\\
    \bottomrule
    \end{tabular}

 %   \vspace{-0.2in}
\end{table}

==> [NeurIPS 2021] Self-Diagnosing GAN/tables/dcgan_generator.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{table}[h]
    \caption{Generator architecture for Colored MNIST \& MNIST-FMNIST}
    \label{table:dcgan_gen}
    \centering
    \small
    \begin{tabular}{c|c|c|c|c|c|c}
    \toprule
    \multicolumn{7}{c}{\textbf{Generator}} \\
    \midrule
    Layer & Output size & Kernel size & Stride & Padding & Batch Norm & Activation  \\
    \midrule
    Input $z$ & 100 & & & & &\\
    FC & 384 & - & - & - & X & \\
    Reshape & 1$\times$1$\times$384 & - & - & - & - & - \\
    Deconv & 4$\times$4$\times$192 & 4$\times$4 & 1 & 0 & O & ReLU \\
    Deconv & 8$\times$8$\times$96 & 4$\times$4 & 2 & 1 & O & ReLU \\
    Deconv & 16$\times$16$\times$48 & 4$\times$4 & 2 & 1 & O & ReLU \\
    Deconv & 32$\times$32$\times$\texttt{nc} & 4$\times$4 & 2 & 1 & X & Tanh \\
    \bottomrule
    \end{tabular}
  %  \vspace{-0.2in}
\end{table}

==> [NeurIPS 2021] Self-Diagnosing GAN/tables/decoder.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{table}[!ht]
    \caption{Decoder architecture for measuring Reconstruction Error (RE) score}
    \label{table:decoder}
    \centering
    \small
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \toprule
    \multicolumn{8}{c}{\textbf{Decoder}} \\
    \midrule
    Layer & Output size & Kernel size & Stride & Padding & Output padding & Batch Norm & Activation \\
    \midrule
    Input $z$ & 256 & & & & & &\\
    FC & (4$\times$4$\times$256) & - & - & - & - & O & ReLU \\
    Reshape & 4$\times$4$\times$256 & - & - & - & - & - & - \\
    Deconv & 8$\times$8$\times$128 & 3$\times$3 & 2 & 1 & 1 & O & ReLU \\
    Deconv & 16$\times$16$\times$64 & 3$\times$3 & 2 & 1 & 1 & O & ReLU \\
    Deconv & 32$\times$32$\times$\texttt{nc} & 3$\times$3 & 2 & 1 & 1 & X & Tanh \\
    \bottomrule
    \end{tabular}

 %   \vspace{-0.2in}
\end{table}

==> [NeurIPS 2021] Self-Diagnosing GAN/tables/encoder.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{table}[t]
    \caption{Encoder architecture for measuring Reconstruction Error (RE) score}
    \label{table:encoder}
    \centering
    \small
    \begin{tabular}{c|c|c|c|c|c|c}
    \toprule
    \multicolumn{7}{c}{\textbf{Encoder}} \\
    %\hline
    \midrule
    Layer & Output size & Kernel size & Stride & Padding & Batch Norm & Activation  \\
    \midrule
    Input $x$ & 32$\times$32$\times$\texttt{nc} &     &   &   &   \\
    Conv & 16$\times$16$\times$64 & 3$\times$3 & 2 & 1 & O & ReLU \\
    Conv & 8$\times$8$\times$128 & 3$\times$3 & 2 & 1 & O & ReLU \\
    Conv & 4$\times$4$\times$256 & 3$\times$3 & 2 & 1 & O & ReLU \\
    Flatten & - & - & - & - & - & - \\
    FC & 256  & - & - & - & X & Tanh\\
    \bottomrule
    \end{tabular}

%    \vspace{-0.2in}
\end{table}

==> [NeurIPS 2021] Self-Diagnosing GAN/tables/hyperparameter.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{table*}[!htb]
    \caption{FID for Dia-GAN with various $k$} 
    \label{Atable:hyperparameter}
    \centering
    \small
    \begin{tabular}{c|c|c|c|c|c|c}
    \toprule
    $k$    & 0.3    & 0.5 & 1.0    & 3.0 & 5.0 & 7.0\\
    \midrule
    FID for CIFAR-10 & \textbf{19.23} & 19.47 & 20.58 & 23.45 & 24.44 & 20.43\\
    \midrule
    FID for CelebA & 7.27 & 6.91 & 6.52 & 6.73 & \textbf{6.37} & 6.41\\
    \bottomrule
    \end{tabular}

\end{table*}


==> [NeurIPS 2021] Self-Diagnosing GAN/tables/hyperparameter_steps.tex <==
\begin{table}[h]
    \caption{FID for Dia-GAN with different phase 1 steps (\% of total steps).}
    \label{Atable:hyperparameter_steps}
    % \small
    \centering
    %\scalebox{0.87}{
    %\tabcolsep=0.11cm
    \small
    \begin{tabular}{c|c|c|c|c|c}
    \toprule
    & \textbf{Baseline} & \textbf{20\%} & \textbf{40\%} & \textbf{60\%} & \textbf{80\%} \\
    \midrule
    % CIFAR-10 & 21.99\scriptsize{$\pm$1.73} & 7.67\scriptsize{$\pm$0.16} & 6.66\scriptsize{$\pm$}0.06 \\
    FID for CIFAR-10 & 26.90\scriptsize{$\pm$0.90} & 17.56\scriptsize{$\pm$1.03} & \textbf{16.72\scriptsize{$\pm$0.74}} & 18.65\scriptsize{$\pm$0.94} & 19.66\scriptsize{$\pm$0.42} \\
    \midrule
    FID for CelebA & 7.12\scriptsize{$\pm$0.27} & \textbf{6.69\scriptsize{$\pm$0.33}} & 6.90\scriptsize{$\pm$0.66} & 6.86\scriptsize{$\pm$0.77} & 6.70\scriptsize{$\pm$0.69}\\
    \bottomrule
    \end{tabular}
    %}

\end{table}

==> [NeurIPS 2021] Self-Diagnosing GAN/tables/longer_training.tex <==
\newcolumntype{?}{!{\vrule width 0.8pt}}

\begin{table}[!tb]
\centering
\caption{FID for SNGAN and Dia-SNGAN with different total training steps.}
\label{table:longer_training}
\vspace{0.2em}
\small
\begin{tabular}{c?c|c?c|c|c}
\toprule
\multirow{2}{*}{} & \multicolumn{2}{c?}{CIFAR-10} & \multicolumn{3}{c}{CelebA} \\
\cmidrule{2-6}
& FID $\downarrow$ & IS $\uparrow$ & FID $\downarrow$ & P $\uparrow$ & R $\uparrow$ \\
\midrule
SNGAN (50k/ 75k) & 26.90\scriptsize{$\pm$0.90} & 7.36\scriptsize{$\pm$0.08} & 7.12\scriptsize{$\pm$0.27} & \textbf{0.68\scriptsize{$\pm$0.00}} & 0.44\scriptsize{$\pm$0.01} \\
Dia-SNGAN (50k/ 75k) & \textbf{19.66\scriptsize{$\pm$0.42}} & \textbf{7.95\scriptsize{$\pm$0.09}} & \textbf{6.70\scriptsize{$\pm$0.69}} & 0.64\scriptsize{$\pm$0.02} & \textbf{0.48\scriptsize{$\pm$0.02}} \\
\midrule
SNGAN (100k) & 22.43\scriptsize{$\pm$0.92} & 7.59\scriptsize{$\pm$0.06} & 6.83\scriptsize{$\pm$0.46} & \textbf{0.68\scriptsize{$\pm$0.00}} & 0.45\scriptsize{$\pm$0.02} \\
Dia-SNGAN (100k) & \textbf{16.49\scriptsize{$\pm$1.05}} & \textbf{8.10\scriptsize{$\pm$0.14}} & \textbf{6.57\scriptsize{$\pm$0.70}} & 0.63\scriptsize{$\pm$0.01} & \textbf{0.49\scriptsize{$\pm$0.01}} \\
\bottomrule
\end{tabular}
\end{table}

==> [NeurIPS 2021] Self-Diagnosing GAN/tables/minor_ldrv.tex <==
\begin{table}[b]
\centering
\caption{Averaged LDRV of major/minor groups on various datasets with majority rate 90\%.}
\label{tab:minor_ldrv}
\vspace{0.2em}
\begin{tabular}{c|ccc}
\toprule
Group &Gaussian ($\sigma$=3.0)  & Colored MNIST & MNIST-FMNIST \\
\midrule
Major & 0.001 & 0.077 & 0.082 \\
Minor & 0.098 & 0.186 & 0.115 \\
\bottomrule
\end{tabular}
%\vspace{-1em}
\end{table}

==> [NeurIPS 2021] Self-Diagnosing GAN/tables/mlp_discriminator.tex <==
\begin{tabular}{c|c|c}
\toprule
\multicolumn{3}{c}{\textbf{Discriminator}} \\
\midrule
Layer & Output size & Activation  \\
\midrule
Input $x$ & 2 & \\
FC & 512 & ReLU\\
FC & 512 & ReLU \\
FC & 512 & ReLU \\
FC & 1 & Sigmoid \\
\bottomrule
\end{tabular}

==> [NeurIPS 2021] Self-Diagnosing GAN/tables/mlp_generator.tex <==
\begin{tabular}{c|c|c}
\toprule
\multicolumn{3}{c}{\textbf{Generator}} \\
\midrule
Layer & Output size & Activation  \\
\midrule
Input $z$ & 2 & \\
FC & 512 & ReLU\\
FC & 512 & ReLU \\
FC & 512 & ReLU \\
FC & 2 &  \\
\bottomrule
\end{tabular}


==> [NeurIPS 2021] Self-Diagnosing GAN/tables/mnist_discriminator.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{table}[!ht]
    \caption{Discriminator architecture for MNIST-FMNIST mixture}
    \label{table:mnist_disc}
    \centering
    \small
    \begin{tabular}{c|c|c|c|c|c|c}
    \specialrule{.1em}{.05em}{.05em}
    \multicolumn{7}{c}{\textbf{Discriminator}} \\
    %\hline
    \specialrule{.1em}{.05em}{.05em}
    Layer & Output size & Kernel size & Stride & Padding & Batch Norm & Activation function \\
    \hline
    Input $x$ & 32$\times$32$\times$3 &     &   &   &   \\
    Conv & 16$\times$16$\times$64 & 4$\times$4 & 2 & 1 & X & LeakyReLU(0.2) \\
    Conv & 8$\times$8$\times$128 & 4$\times$4 & 2 & 1 & O & LeakyReLU(0.2) \\
    Flatten & - & - & - & - & - & - \\
    FC & 1024 & - & - & - & O & LeakyReLU(0.2) \\
    FC & 1  & - & - & - & X & Sigmoid\\
    \specialrule{.1em}{.05em}{.05em}
    \end{tabular}

%    \vspace{-0.2in}
\end{table}

==> [NeurIPS 2021] Self-Diagnosing GAN/tables/mnist_generator.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{table}[!ht]
    \caption{Generator architecture for MNIST-FMNIST mixture}
    \label{table:mnist_gen}
    \centering
    \small
    \begin{tabular}{c|c|c|c|c|c|c}
    \specialrule{.1em}{.05em}{.05em}
    \multicolumn{7}{c}{\textbf{Generator}} \\
    \specialrule{.1em}{.05em}{.05em}
    Layer & Output size & Kernel size & Stride & Padding & Batch Norm & Activation function \\
    \hline
    Input $z$ & 100 & & & & &\\
    FC & 1024 & - & - & - & O & ReLU \\
    FC & (8$\times$8$\times$128) & - & - & - & O & ReLU \\
    Reshape & 8$\times$8$\times$128 & - & - & - & - & - \\
    Deconv & 16$\times$16$\times$64 & 4$\times$4 & 2 & 1 & O & ReLU \\
    Deconv & 32$\times$32$\times$3 & 4$\times$4 & 2 & 1 & X & Tanh \\
    \specialrule{.1em}{.05em}{.05em}
    \end{tabular}

 %   \vspace{-0.2in}
\end{table}

==> [NeurIPS 2021] Self-Diagnosing GAN/tables/partial_fid.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{comment}
\begin{table}[!ht]
    \caption{Partial FID for SNGAN}
    \label{table:fid_with_index}
    \centering
    \small
    \begin{tabular}{c|c|c|c}
    \specialrule{.1em}{.05em}{.05em}
    \multicolumn{2}{c|}{} & Baseline & Dia-GAN (ours) \\
    \hline
    \multirow{2}{*}{CIFAR-10} & High PFID & {94.64}\scriptsize{$\pm$2.93} & 77.28\scriptsize{$\pm$3.76}\\
    & Low PFID & 22.43\scriptsize{$\pm$0.68} & 33.98\scriptsize{$\pm$1.77}\\
    \hline
    \multirow{2}{*}{CelebA} & High PFID & 50.25\scriptsize{$\pm$3.24} & 42.33\scriptsize{$\pm$3.36}\\
    \cline{2-4}
    & Low PFID & 17.25\scriptsize{$\pm$1.35} & 23.17\scriptsize{$\pm$3.29}\\
    \specialrule{.1em}{.05em}{.05em}
    \end{tabular}

 %   \vspace{-0.2in}
\end{table}
\end{comment}

\begin{table}[!ht]
    \caption{Partial FID for SNGAN}
    \label{table:fid_with_index}
    \centering
    \small
    \begin{tabular}{c|c|c|c}
    \toprule
    \multicolumn{2}{c|}{} & Baseline & Dia-GAN (ours) \\
    \midrule
    \multirow{2}{*}{CIFAR-10} & High PFID & {94.64}\scriptsize{$\pm$2.93} & 77.28\scriptsize{$\pm$3.76}\\
    \cmidrule{2-2} \cmidrule{3-4}
    & Low PFID & 22.43\scriptsize{$\pm$0.68} & 33.98\scriptsize{$\pm$1.77}\\
    \midrule
    \multirow{2}{*}{CelebA} & High PFID & 50.25\scriptsize{$\pm$3.24} & 42.33\scriptsize{$\pm$3.36}\\
    \cmidrule{2-2} \cmidrule{3-4}
    & Low PFID & 17.25\scriptsize{$\pm$1.35} & 23.17\scriptsize{$\pm$3.29}\\
    \bottomrule
    \end{tabular}

 %   \vspace{-0.2in}
\end{table}

==> [NeurIPS 2021] Self-Diagnosing GAN/tables/simple_convnet.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{table}[t]
    \caption{Classifier architecture for measuring Partial Recall of Colored MNIST \& MNIST-FMNIST}
    \label{table:convnet}
    \centering
    \small
    \begin{tabular}{c|c|c|c|c|c|c}
    \toprule
    \multicolumn{7}{c}{\textbf{Classifier}} \\
    %\hline
    \midrule
    Layer & Output size & Kernel size & Stride & Padding & Batch Norm & Activation  \\
    \midrule
    Input $x$ & 32$\times$32$\times$\texttt{nc} &     &   &   &   \\
    Conv & 32$\times$32$\times$16 & 7$\times$7 & 1 & 3 & O & ReLU \\
    Conv & 32$\times$32$\times$32 & 7$\times$7 & 1 & 3 & O & ReLU \\
    Conv & 32$\times$32$\times$64 & 7$\times$7 & 1 & 3 & O & ReLU \\
    Conv & 32$\times$32$\times$128 & 7$\times$7 & 1 & 3 & O & ReLU \\
    AvgPool & 1$\times$1$\times$128 & - & - & - & - & - \\
    Flatten & - & - & - & - & - & - \\
    FC & 20  & - & - & - & X & Softmax\\
    \bottomrule
    \end{tabular}

%    \vspace{-0.2in}
\end{table}

==> [NeurIPS 2021] Self-Diagnosing GAN/tables/stylegan_hingegan.tex <==
\begin{table}[t]
%\caption{Global caption}
\begin{minipage}{.45\linewidth}
    \caption{StyleGAN2 on FFHQ 256x256.}
    \label{tab:stylegan2}
    \vspace{0.2em}
    \centering
    \begin{tabular}{c|ccc}
        \toprule
        %& StyleGAN2 & \textbf{Dia-StyleGAN2}  \\
        %\midrule
        %FID $\downarrow$ & 14.07 & \textbf{11.89} \\
        & FID $\downarrow$ & P $\uparrow$   & R $\uparrow$ \\
        \midrule
        StyleGAN2 & 14.07   & \textbf{0.72}  & 0.27 \\
        GOLD    & 15.53 & 0.69  & 0.29 \\
        \textbf{Dia-StyleGAN2}  & \textbf{11.89} & 0.69  & \textbf{0.30} \\
        \bottomrule
    \end{tabular}
\end{minipage} 
\begin{minipage}{.53\linewidth}
    \caption{HingeGAN on CIFAR-10 and CelebA.}
    \label{table:hingegan}
    \vspace{0.2em}
    \centering
    %\scalebox{0.87}{
    %\tabcolsep=0.11cm

    %\small
    %\begin{tabular}{cc|cc}
    
    %\toprule
    %      &  & HingeGAN &  \textbf{Dia-HingeGAN}  \\
    %\midrule
    %\multirow{2}{*}{CIFAR-10} & FID $\downarrow$ & 21.99 & \textbf{18.74}\\
    %  & IS $\uparrow$  & 7.67& \textbf{8.02} \\
    %  \midrule
    %CelebA & FID $\downarrow$  & 6.66& \textbf{5.98}\\
    %\bottomrule
    %\end{tabular}
    
    \begin{tabular}{c|cc|c}
    \toprule \label{tab:hingeGAN}
    \multirow{2}{*}{}     &  \multicolumn{2}{c|}{CIFAR-10} & CelebA\\
    \cmidrule{2-4}
    & FID $\downarrow$ & IS $\uparrow$ & FID $\downarrow$\\
    \midrule
    HingeGAN & 21.99 & 7.67 & 6.66\\
    \textbf{Dia-HingeGAN} & \textbf{18.74} & \textbf{8.02} & \textbf{5.98}\\
    \bottomrule
    \end{tabular}

\end{minipage}
\end{table}

==> figures/color_mnist_samples_arxiv.tex <==
\begin{figure}[t]
    \subfloat[Training data \label{fig:color_mnist_samples_train}]{\includegraphics[width=0.315\linewidth]{{figures/color_mnist_train.jpg}}}
	\hspace{0.3em}
    \centering
	\subfloat[PacGAN\label{fig:color_mnist_samples_PAC}]{\includegraphics[width=0.315\linewidth]{{figures/color_mnist_pacgan_gen.jpg}}}
	\hspace{0.3em}
    \subfloat[DiaGAN (Ours) \label{fig:color_mnist_samples_ours}]{\includegraphics[width=0.315\linewidth]{{figures/color_mnist_diagan_gen.jpg}}}
    \caption{Generated samples in Colored-MNIST with the majority rate of 99\%. (a) Examples of training data (b) Samples from PacGAN. (c) Dia-GAN (Ours). Our method successfully generates samples with minor features, while  others fail, as in (b).}
    \label{fig:color_mnist_samples}
\end{figure}

==> figures/ldr_instability.tex <==
\begin{figure}[t]
    \centering
    \subfloat[\label{fig:LDR_instability}]{\includegraphics[width=0.35\linewidth]{{figures/ldr_eval_3idx.png}}} 
	\subfloat[\label{fig:LDR_plot}]{\includegraphics[width=0.65\linewidth]{{figures/ldr_instability2.png}}}
	\caption{(a) LDR values of three randomly chosen samples, (b) LDR values (left) and rankings (right) of 50 samples during training of CIFAR-10 on SNGAN~\cite{sngan}. The values are recorded every 100 steps from 30000 to 40000 epochs (total 100 times). LDR values are unstable during training, so it is hard to diagnose GAN training from the LDR of a particular training step. The level of fluctuations varies much over samples. %We propose to use statistics of 
	}\label{fig:LDR_inst}
\end{figure}

==> tables/LDRV_detection.tex <==
\begin{table}[]
    \caption{AUROC of minority detection using LDRM and LDRV on Colored-MNIST with various majority rates.}
    % \small
    % \vspace{-0.5em}
    \centering
    %\scalebox{0.87}{
    %\tabcolsep=0.11cm
    \small
    \begin{tabular}{c|c|c|c|c}
    \specialrule{.1em}{.05em}{.05em}
    Majority rate & \textbf{99\%} & \textbf{97\%} & \textbf{95\%} & \textbf{90\%} \\
    \hline
    LDRM & \textbf{1.000} & 0.327 & 0.418  & 0.566\\
    \hline
    LDRV & 0.172 & \textbf{0.997} & \textbf{0.999} & \textbf{0.992}\\
    \specialrule{.1em}{.05em}{.05em}
    \end{tabular}
    %}
   % \vspace{-0.5\baselineskip}

    \label{table:ldrv_detection}
%    \vspace{-0.5em}
\end{table}

==> tables/mnist_discriminator.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{table}[!ht]
    \caption{Discriminator architecture for MNIST-FMNIST mixture}
    \label{table:mnist_disc}
    \centering
    \small
    \begin{tabular}{c|c|c|c|c|c|c}
    \specialrule{.1em}{.05em}{.05em}
    \multicolumn{7}{c}{\textbf{Discriminator}} \\
    %\hline
    \specialrule{.1em}{.05em}{.05em}
    Layer & Output size & Kernel size & Stride & Padding & Batch Norm & Activation function \\
    \hline
    Input $x$ & 32$\times$32$\times$3 &     &   &   &   \\
    Conv & 16$\times$16$\times$64 & 4$\times$4 & 2 & 1 & X & LeakyReLU(0.2) \\
    Conv & 8$\times$8$\times$128 & 4$\times$4 & 2 & 1 & O & LeakyReLU(0.2) \\
    Flatten & - & - & - & - & - & - \\
    FC & 1024 & - & - & - & O & LeakyReLU(0.2) \\
    FC & 1  & - & - & - & X & Sigmoid\\
    \specialrule{.1em}{.05em}{.05em}
    \end{tabular}

%    \vspace{-0.2in}
\end{table}

==> tables/mnist_generator.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{table}[!ht]
    \caption{Generator architecture for MNIST-FMNIST mixture}
    \label{table:mnist_gen}
    \centering
    \small
    \begin{tabular}{c|c|c|c|c|c|c}
    \specialrule{.1em}{.05em}{.05em}
    \multicolumn{7}{c}{\textbf{Generator}} \\
    \specialrule{.1em}{.05em}{.05em}
    Layer & Output size & Kernel size & Stride & Padding & Batch Norm & Activation function \\
    \hline
    Input $z$ & 100 & & & & &\\
    FC & 1024 & - & - & - & O & ReLU \\
    FC & (8$\times$8$\times$128) & - & - & - & O & ReLU \\
    Reshape & 8$\times$8$\times$128 & - & - & - & - & - \\
    Deconv & 16$\times$16$\times$64 & 4$\times$4 & 2 & 1 & O & ReLU \\
    Deconv & 32$\times$32$\times$3 & 4$\times$4 & 2 & 1 & X & Tanh \\
    \specialrule{.1em}{.05em}{.05em}
    \end{tabular}

 %   \vspace{-0.2in}
\end{table}
